Does Fair Ranking Improve Minority Outcomes? Understanding the Interplay of Human and Algorithmic Biases in Online Hiring

Ranking algorithms are being widely employed in various online hiring platforms including LinkedIn, TaskRabbit, and Fiverr. Prior research has demonstrated that ranking algorithms employed by these platforms are prone to a variety of undesirable biases, leading to the proposal of fair ranking algorithms (e.g., Det-Greedy) which increase exposure of underrepresented candidates. However, there is little to no work that explores whether fair ranking algorithms actually improve real world outcomes (e.g., hiring decisions) for underrepresented groups. Furthermore, there is no clear understanding as to how other factors (e.g., job context, inherent biases of the employers) may impact the efficacy of fair ranking in practice. In this work, we analyze various sources of gender biases in online hiring platforms, including the job context and inherent biases of employers and establish how these factors interact with ranking algorithms to affect hiring decisions. To the best of our knowledge, this work makes the first attempt at studying the interplay between the aforementioned factors in the context of online hiring. We carry out a largescale user study simulating online hiring scenarios with data from TaskRabbit, a popular online freelancing site. Our results demonstrate that while fair ranking algorithms generally improve the selection rates of underrepresented minorities, their effectiveness relies heavily on the job contexts and candidate profiles.

==> 06-acknowledgements.tex <==
\section{Acknowledgements}
 


==> 08-limitations.tex <==
\section{Limitations}\label{sec:limitations}
\hima{Don't worry about this section at all. Remove this completely. Just add a few limitations under the guise of "Future Work" in Conclusions Section.}

==> 09-fairness.tex <==
\section{Fairness in Rankings}\label{sec:fairness}
Fair ranking algorithms try to achieve a fair distribution of click probability among groups or individuals.
\subsection{Individual Fairness}\label{subsec:indfairness}
\begin{itemize}
\item Explain equity of attention \citep{biega2018equity} as notion of individual fairness of attention in rankings
\end{itemize}
\subsection{Group Fairness}\label{subsec:groupfairness}
\begin{itemize}
\item Explain notions of group fairness like in \cite{zehlike2017fa}, \cite{singh2018fairness}
\end{itemize}

